Large Language Model-Aware In-Context Learning for Code Generation

Large language models (LLMs) have shown impressive in-context learning (ICL) ability in code generation. LLMs take a prompt consisting of requirement-code examples and a new requirement as input, and output new programs. Existing studies have found that ICL is highly dominated by the examples and thus arises research on example selection. However, existing approaches randomly select examples or only consider the textual similarity of requirements to retrieve, leading to sub-optimal performance. In this paper, we propose a novel learning-based selection approach named LAIL (LLM-Aware In-context Learning) for code generation. Given a candidate example, we exploit LLMs themselves to estimate it by considering the generation probabilities of ground-truth programs given a requirement and the example. We then label candidate examples as positive or negative through the probability feedback. Based on the labeled data, we import a contrastive learning objective to train an effective retriever that acquires the preference of LLMs in code generation. We apply LAIL to three LLMs and evaluate it on three representative datasets (e.g., MBJP, MBPP, and MBCPP). LATA outperforms the state-of-the-art baselines by 11.58%, 6.89%, and 5.07% on CodeGen, and 4.38%, 2.85%, and 2.74% on GPT-3.5 in terms of Pass@1, respectively.

==> main_cf.tex <==
\section{introduction}

Code generation aims to automatically generate the source code given a natural language requirement. Code generation is an important part of automated software engineering and has attracted the attention of many researchers. 

In-context learning (ICL) is a recent paradigm with large language models (LLMs) in code generation and achieves state-of-the-art performance\cite{fried2022incoder, zhong2022codegen, AlphaCode, li2023towards}. ICL does not require training and directly performs inference using LLMs. In ICL, developers construct a prompt for LLMs to generate codes. The prompt consists of two components: (1) a few requirement-code examples, and (2) a test input requirement. Previous works have shown ICL strongly relies on the provided examples and randomly sampled examples are significantly unstable in performance \cite{zhao2021calibrate, li2023towards, li2023finding}. Therefore, it is necessary to investigate how to select examples for ICL in code generation.

Recently, some works \cite{li2023towards} have made some attempts in code generation. 
The straightforward method is randomly sampling some examples from the training set.

%用户通过输入prompt来利用LLMs生成代码。一个prompt包含两部分：（1）examples，requirement-code pairs；（2）Input requirement
%现有研究表明：examples对LL。Ms的性能有较大的影响。
%因此，有必要研究standard ，在代码生成任务上，如何挑选examples。
%已经有一些工作做了这方面的尝试：AceCoder...
%但它们仅仅从文本相似度的层面去检索相似examples。检索出的examples在语义上可能与input requirement不相关。【citation】



%Given a specific requirement, we take a candidate example and the requirement as input and estimate the probability of its ground-truth code provided by LLMs. We label candidate examples as positive and negative examples based on their probabilities. We then train a example retriever from the label data. In the test, we use the trained retriever to select examples given a test requirement, and prompt LLMs to generate codes.
